The clustering of the SDSS-IV extended Baryon Oscillation Spectroscopic Survey quasar sample: Testing observational systematics on the Baryon Acoustic Oscillation measurement

Baryon Acoustic Oscillations are considered to be a very robust standard ruler against various systematics. This premise has been tested against observational systematics, but not to the level required for the next generation of galaxy surveys such as the Dark Energy Spectroscopic Instrument (DESI) and Euclid. In this paper, we investigate the effect of observational systematics on the BAO measurement of the final sample of quasars from the extended Baryon Oscillation Spectroscopic Survey Data Release 16 in order to prepare and hone a similar analysis for upcoming surveys. We employ catalogues with various treatments of imaging systematic effects using linear and neural network-based nonlinear approaches and consider how the BAO measurement changes. We also test how the variations to the BAO fitting model respond to the observational systematics. As expected, we confirm that the BAO measurements obtained from the DR16 quasar sample are robust against imaging systematics well within the statistical error, while reporting slightly modified constraints that shift the line-of-sight BAO signal by less than 1.1% . We use realistic simulations with similar redshift and angular distributions as the DR16 sample to conduct statistical tests for validating the pipeline, quantifying the significance of differences, and estimating the expected bias on the BAO scale in future high-precision data sets. Although we find a marginal impact for the eBOSS QSO data, the work presented here is of vital importance for constraining the nature of dark energy with the BAO feature in the new era of big data cosmology with DESI and Euclid.

==> Grant's BAO Paper (Version 9573)/tables/tab1.tex <==
 \renewcommand*{\thefootnote}{\fnsymbol{footnote}}

\begin{table*}

      \caption{The BAO constraints from the eBOSS QSO catalog using different mitigation methods. `Default' here presents our reproduction of the \citet{Neveux20} using exactly the same setup. 
      Posterior values are taken as the mean and standard deviation of the MCMC chains.  Shifts $\Delta\alpha$ are compared to the default fit. Catalogs are grouped by the HEALPIX resolution used to determine NN weights.  Values in parentheses are derived from chi-square minimization rather than the posterior mean.}
      \label{tab:alphatable}

    \begin{threeparttable}
        \begin{adjustbox}{max width=\textwidth}

         \begin{tabular}{ l | l  l  l  l  l  l  l  l}%{\textwidth}
 & $\alpha_\parallel$ & $\Delta \alpha_\parallel $ & $\alpha_\perp$ &  $\Delta \alpha_\perp$ & $r_{\rm off}$  &$\alpha_{\rm iso}$ & $\Delta\alpha_{\rm iso}$  &$\chi^2$\\
 \hline
   Neveux 2020\tnote{*} & 1.035 $\pm$ 0.045 & -- & 1.017 $\pm$ 0.029 & -- & --  & --- & --- & 87.63 / 104 \\
  \hline
  default & 1.0386 (1.0361) $\pm$ 0.0528 & -- & 1.0169(1.0141) $\pm$ 0.0328 & -- & -0.3923 & 1.0236 (1.0214) $\pm$ 0.0215 & -- & (88.910) / 104 \\
  \hline
  no wsys & 1.0324 (1.0303) $\pm$ 0.0524 & -0.0062 (-0.0058) & 1.0165 (1.0131) $\pm$ 0.0343 & -0.0004 (-0.0009) & -0.3828 & 1.0212 (1.0188) $\pm$ 0.0224 & -0.0024  (-0.0025) & (90.823)/104\\
  \hline
  H512 & & & & &\\
  known-1z & 1.0307 (1.0273) $\pm$ 0.0550 & -0.0079 (-0.0089) &  1.0139 (1.0110) $\pm$ 0.0348 &  -0.0030 (-0.0030) & -0.3890 & 1.0189 (1.0164) $\pm$ 0.0228  & -0.0047 (-0.0050) & (91.082)/104 \\
  known-1z\tnote{\textdagger} & 1.0292 (1.0255) $\pm$ 0.0532 & -0.0095 (-0.0107) &  1.0166 (1.0139) $\pm$ 0.0342 &  -0.0003 (-0.0002) & -0.3977 & 1.0202 (1.0177) $\pm$ 0.0222 & -0.0034 (-0.0036) & (92.861)/104 \\
  known-2z & 1.0322 (1.0284) $\pm$ 0.0545 & -0.0064 (-0.0077) & 1.0130 (1.0102) $\pm$ 0.0348 & -0.0039 (-0.0039) & -0.3716 & 1.0188 (1.0162) $\pm$ 0.0230  & -0.0048 (-0.0051)  & (91.004)/104 \\
  all-1z & 1.0321 (1.0283) $\pm$ 0.0538 & -0.0066 (-0.0078) & 1.0125 (1.0113) $\pm$ 0.0342  & -0.0044 (-0.0027) & -0.3547 & 1.0184 (1.0169) $\pm$ 0.0230 & -0.0051 (-0.0044)  &  (91.011)/104 \\
  all-2z & 1.0361 (1.0323) $\pm$ 0.0544 & -0.0025 (-0.0038) & 1.0108 (1.0083) $\pm$ 0.0339 & -0.0061 (-0.0057) &  -0.4065 &  1.0186 (1.0163) $\pm$ 0.0220 & -0.0050 (-0.0051) & (91.178)/104 \\
  \hline
  H256 & & & & &\\
  known-1z & 1.0318 (1.0282) $\pm$ 0.0560 & -0.0068  (-0.0079) &  1.0144 (1.0108) $\pm$ 0.0343 &  -0.0025 (-0.0033) & -0.3805 & 1.0196 (1.0165) $\pm$ 0.0229 & -0.0040 (-0.0048) & (92.571)/104 \\
  known-2z & 1.0310 (1.0281)  $\pm$ 0.0539 & -0.0076 (-0.0080) & 1.0138 (1.0103)  $\pm$ 0.0345 & -0.0031 (-0.0038) &  -0.4008  & 1.0189  (1.0162) $\pm$ 0.0223 & -0.0046 (-0.0052) &  (90.247)/104 \\
  all-1z & 1.0341 (1.0302) $\pm$ 0.0540 & -0.0045 (-0.0059) &  1.0133 (1.0109) $\pm$ 0.0343 & -0.0036 (-0.0032) & -0.3627 & 1.0196 (1.0173) $\pm$ 0.0229 & -0.0039 (-0.0041) &  (91.094)/104 \\
  all-2z & 1.0349 (1.0304) $\pm$ 0.0537 & -0.0038 (-0.0057) & 1.0113 (1.0095) $\pm$ 0.0347 & -0.0055 (-0.0045) &  -0.3874 & 1.0186 (1.0164) $\pm$ 0.0226 & -0.0050 (-0.0049)  & (91.749) /104 \\
\hline
    \end{tabular}
    \end{adjustbox}
    \begin{tablenotes}
    \item[*] Error is derived from the $\Delta\chi^2=1$ abscissa
    \item[\textdagger] Fit performed using a covariance matrix derived from mocks with the same NN mitigation
    \end{tablenotes}
    \end{threeparttable}

\end{table*}


==> Grant's BAO Paper (Version 9573)/tables/tab2.tex <==
\begin{table*}
\centering
\caption{The BAO constraints from the eBOSS QSO catalog using the default and the NN mitigation methods when the BAO fitting parameters are varied. As in Table \ref{tab:alphatable}, `default' presents our reproduction of the \citet{Neveux20} using exactly the same setup. 
%Results of the fitting the catalogs with a slightly different model.  
Listed are fits of the default catalog with default covariance, and the known-512-1z catalog with covariance derived from the same NN setup.  Shifts $\Delta\alpha$ in the default rows are compared to the default fit with the standard model.  Shifts $\Delta\alpha$ in the `known' rows are compared to the default fit with the same model.  We compare a model with $f$ as a free parameter and a model with an additional $k^{-2}$ polynomial. }
\normalsize
\resizebox{\textwidth}{!}{% use resizebox with textwidth
\begin{tabular}{ l | l  l  l  l  l  l  l  l}
 & $\alpha_\parallel$ & $\Delta \alpha_\parallel$ & $\alpha_\perp$ & $\Delta \alpha_\perp$ & $r_{\rm off}$ & $\alpha_{\rm iso}$ & $\Delta\alpha_{\rm iso}$ & $\chi^2$ / dof\\
  \hline
   Neveux 2020 & (1.035) $\pm$ 0.045 & -- & (1.017) $\pm$ 0.029 & -- & -- & -- & -- & 87.63 / 104 \\
  \hline
  default & 1.0386 (1.0361) $\pm$ 0.0528 & -- & 1.0169(1.0141) $\pm$ 0.0328 & -- & -0.3923 & 1.0236 $\pm$ 0.0215 & -- & (88.910)/104 \\
  default (free f) & 1.0465 (1.0493) $\pm$  0.0500 & 0.0087 (0.0132) & 1.0112 (1.0024) $\pm$ 0.0343 & -0.0058 (-0.0117) &  -0.3700 & 1.0223 (1.0178) $\pm$ 0.0223 & -0.0012 (-0.0036) & (87.266) / 103 \\
  default ($k^{-2}$) & 1.0320 (1.0295) $\pm$  0.0458 & -0.0058 (-0.0066) & 1.0182 (1.0160) $\pm$ 0.0281 & 0.0011 (0.0019) &  -0.3870 & 1.0223 (1.0204) $\pm$ 0.0186 & -0.0012 (-0.0009) & (80.815) / 98 \\
  default (no $\ell=4$) & 1.0457 (1.0415) $\pm$ 0.0545 & 0.0070 (0.0053) & 1.0181 (1.0154) $\pm$ 0.0341 & 0.0012 (0.0013) & -0.4167 & 1.0266 (1.0240) $\pm$ 0.0219 & 0.0031 (0.0027) & (47.346) / 68 \\
  \hline
   known & 1.0292 (1.0255) $\pm$ 0.0532 & -0.0095 (-0.0107) & 1.0166 (1.0139) $\pm$ 0.0342 & -0.0003 (-0.0002) & -0.3977 & 1.0202 (1.0177) $\pm$ 0.0222 & -0.0034 (-0.0036)  & (92.861) / 104\\
  known (free f) & 1.0408 (1.0377) $\pm$ 0.0494 & -0.0057 (-0.0116) & 1.0097 (1.0031) $\pm$ 0.0338 & -0.0015 (0.0008) & -0.3706 & 1.0195 (1.0145) $\pm$ 0.0220 & -0.0029 (-0.0033) & (89.572) / 103\\
  known ($k^{-2}$) & 1.0204 (1.0180) $\pm$  0.0436 & -0.0115 (-0.0115) & 1.0188 (1.0171) $\pm$ 0.0287 & 0.0006 (0.0011) &  -0.3656 & 1.0189 (1.0174) $\pm$ 0.0189 & -0.0034 (-0.0031)  & (82.044) / 98 \\
  known (no $\ell$=4) & 1.0321 (1.0272) $\pm$  0.0567 & -0.0135 (-0.0143) & 1.0183 (1.0150) $\pm$ 0.0347 & 0.0002 (-0.0004) &  -0.4253 & 1.0223 (1.0190) $\pm$ 0.0223 & -0.0044 (-0.0050) & (56.351) / 68 \\\hline
\end{tabular}
}
\label{tab:modeltable}
\end{table*}


==> Grant's BAO Paper (Version 9573)/tables/tab3.tex <==
\begin{table}
\centering
\caption[h]{Results of fitting with the highz sample.  We examine the case of catalogs treated with the known-1z-H512 mitigation and calculate spectra for the standard sample and the standard+highz sample for each galactic cap.}
\resizebox{1.0\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{ l |  l  l  l }
 & $\alpha_\parallel$ & $\alpha_\perp$ & $\chi^2$ / dof\\
  \hline
   NGC & & & \\
   main & 1.016 $\pm$ 0.0788 &  1.009 $\pm$ 0.0367  & 41.14 / 50 \\
   combined & 0.9976 $\pm$ 0.0712 & 1.019 $\pm$ 0.0370 & 46.13 / 50 \\
   \hline
   SGC & & & \\
   main & 1.054 $\pm$ 0.0606 &  1.017 $\pm$ 0.0909  & 45.24 / 50 \\
   combined & 1.040 $\pm$ 0.0539 & 1.000 $\pm$ 0.0719 & 46.10 / 50 \\
   \hline
   NGC+SGC & & & \\
   main & 1.030 $\pm$ 0.0552 &  1.014 $\pm$ 0.0336  & 90.80 / 102 \\   
   combined & 1.012 $\pm$ 0.050 &  1.018 $\pm$ 0.0299  & 94.91 / 102 \\  
   \hline

\end{tabular}% close resizebox
}
\label{tab:highztable}
\end{table}


==> Grant's BAO Paper (Version 9573)/tables/tab4.tex <==
\begin{table}
\centering
\caption{Median shifts and 68\% ranges around the median in the difference in $\alpha$ when fitting to contaminated/null and NN/sys\_tot weighted EZ mocks. The baseline reference is taken to be null mocks with without systematic mitigation, i.e ground truth mocks.}
\normalsize
\resizebox{1.0\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{ l | c  c  c  c }

 baseline: null & <$\Delta\alpha_\parallel$> (\%) & $ <\Delta\alpha_\perp$> (\%)   & $r_{\rm off}(\alpha_\parallel)$  & $r_{\rm off}(\alpha_\perp)$ \\ 
 \hline
  sys\_tot contam &  $-0.096 \pm  0.173 $  & $ 0.021 \pm 0.142 $ &  0.759  & 0.647  \\
  known null &   $ -0.069 \pm 0.113 $ & $ 0.169 \pm 0.088$ &  0.883
  &  0.871  \\
  known contam &  $ -0.197 \pm 0.171 $ & $ 0.149 \pm 0.140 $ & 0.678 &  0.770 \\
  noweight contam &  $ -0.127 \pm 0.115 $ & $ -0.031 \pm 0.140 $ & 0.506 & 0.653 \\
  \hline  

\end{tabular}% close resizebox
}
\label{tab:alphashift}
\end{table}

NN, contam
default
NN, null
contam, no weight

Relative to null sys_tot (ground truth)
apar
0.011569487626905683 +/- [0.24436773 0.22665174]
-0.07366002080733125 +/- [0.23648763 0.22690789]
-6.940277930134187e-06 +/- [0.11187177 0.10279328]
0.00999973264396159 +/- [0.19959853 0.22847554]


aper
0.08388423184167992 +/- [0.16504684 0.16688782]
0.016823116081909895 +/- [0.16027468 0.16612681]
0.14818153577905724 +/- [0.08140876 0.07306003]
-0.10764608590896341 +/- [0.15945608 0.1620402 ]


==> Grant's BAO Paper (Version 9573)/tables/tabNN.tex <==
\begin{table}
\centering
\caption{Labelling conventions and the corresponding NN setup. The default label indicates the linear regression used in \citet{Ross2020}. The bolded label indicates our benchmark NN setup.}

\normalsize
\resizebox{1.0\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{ c | c  c  c}
 label & input templates & zsplit & \textsc{healpix nside}\\
 \hline
 \hline
 default &  PSF$_i$, Sky$_i$, EBV, depth$_g$   & 1  &  512 \\
 \hline
  \textbf{known-1z-H512} &  PSF$_i$, Sky$_i$, EBV, depth$_g$, NStar   & 1  &  512 \\
  known-2z-H512 &  PSF$_i$, Sky$_i$, EBV, depth$_g$, NStar   & 2  &  512 \\
  all-1z-H512 &  PSF$_i$, Sky$_i$, EBV, depth$_g$, NStar + 12 maps & 1  &  512 \\
  all-2z-H512 &  PSF$_i$, Sky$_i$, EBV, depth$_g$, NStar + 12 maps & 2  &  512 \\
  known-1z-H256 &  PSF$_i$, Sky$_i$, EBV, depth$_g$, NStar   & 1  &  256 \\
  known-2z-H256 &  PSF$_i$, Sky$_i$, EBV, depth$_g$, NStar   & 2  &  256 \\
  all-1z-H256 &  PSF$_i$, Sky$_i$, EBV, depth$_g$, NStar + 12 maps & 1  &  256 \\
  all-2z-H256 &  PSF$_i$, Sky$_i$, EBV, depth$_g$, NStar + 12 maps & 2  &  256 \\
  \hline
\end{tabular}% close resizebox
}
\label{tab:NNlabels}
\end{table}

==> Grant's BAO Paper (Version 9573)/tables/tabmocktest.tex <==
\begin{comment}
\begin{table}
\centering
\caption{Median shifts and the error on the median (i.e., 68\% ranges around the median in the difference in $\alpha$ divided by the number of mocks) when fitting to contaminated/null and NN/sys\_tot weighted EZ mocks. The baseline reference is taken to be null mocks with without systematic mitigation, i.e ground truth mocks.}
\normalsize
\resizebox{1.0\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{ l | c  c  c  c }

 baseline: null & <$\Delta\alpha_\parallel$> (\%) & $ <\Delta\alpha_\perp$> (\%)   & $r_{\rm off}(\alpha_\parallel)$  & $r_{\rm off}(\alpha_\perp)$ \\ 
 \hline
  sys\_tot contam &  $-0.074^{+0.227}_{-0.236} $  & $ 0.017^{+0.166}_{-0.160} $ &  0.759  & 0.647  \\[.3cm]
  known null &   $ 0.000^{+0.103}_{-0.112} $ & $ 0.148^{+0.073}_{-0.081} $ &  0.883
  &  0.871  \\[.3cm]
  known contam &  $ 0.012^{+0.227}_{-0.244}$ & $ 0.084^{+0.167}_{-0.165}$ & 0.678 &  0.770 \\[.3cm]
  noweight contam &  $ 0.010^{+0.228}_{-0.200}$ & $ -0.108 ^{+0.162}_{-0.159}$ & 0.506 & 0.653 \\[.3cm]
  \hline  

\end{tabular}% close resizebox
}
\label{tab:alphashift}
\end{table}
\end{comment}






\begin{table}
\centering
\caption{Median shifts and the error on the median (i.e., 68\% ranges around the median in the difference in $\alpha$ divided by the number of mocks) when fitting to contaminated/null and NN/sys\_tot weighted EZ mocks. The baseline reference is taken to be null mocks with without systematic mitigation, i.e ground truth mocks.}
\normalsize
\resizebox{1.0\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{ l | c  c  c  c }

 baseline: null & $<\Delta\alpha_\parallel>$ (\%) & $ <\Delta\alpha_\perp>$ (\%)   & $r_{\rm off}(\alpha_\parallel)$  & $r_{\rm off}(\alpha_\perp)$ \\ 
 \hline
  sys\_tot contam &  $-0.150^{+0.217}_{-0.212} $  & $ 0.049^{+0.163}_{-0.153} $ &  0.759  & 0.647  \\[.3cm]
  known null &   $ -0.049^{+0.109}_{-0.108} $ & $ 0.155^{+0.073}_{-0.080} $ &  0.883
  &  0.871  \\[.3cm]
  known contam &  $ 0.070^{+0.226}_{-0.198}$ & $ 0.115^{+0.157}_{-0.157}$ & 0.678 &  0.770 \\[.3cm]
  noweight contam &  $ 0.053^{+0.217}_{-0.196}$ & $ -0.093 ^{+0.158}_{-0.151}$ & 0.506 & 0.653 \\[.3cm]
  \hline  


\end{tabular}% close resizebox
}
\label{tab:alphashift}
\end{table}


==> tables/tab4.tex <==
\begin{table}
\centering
\caption{Median shifts and 68\% ranges around the median in the difference in $\alpha$ when fitting to contaminated/null and NN/sys\_tot weighted EZ mocks. The baseline reference is taken to be null mocks with without systematic mitigation, i.e ground truth mocks.}
\normalsize
\resizebox{1.0\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{ l | c  c  c  c }

 baseline: null & <$\Delta\alpha_\parallel$> (\%) & $ <\Delta\alpha_\perp$> (\%)   & $r_{\rm off}(\alpha_\parallel)$  & $r_{\rm off}(\alpha_\perp)$ \\ 
 \hline
  sys\_tot contam &  $-0.096 \pm  0.173 $  & $ 0.021 \pm 0.142 $ &  0.759  & 0.647  \\
  known null &   $ -0.069 \pm 0.113 $ & $ 0.169 \pm 0.088$ &  0.883
  &  0.871  \\
  known contam &  $ -0.197 \pm 0.171 $ & $ 0.149 \pm 0.140 $ & 0.678 &  0.770 \\
  noweight contam &  $ -0.127 \pm 0.115 $ & $ -0.031 \pm 0.140 $ & 0.506 & 0.653 \\
  \hline  

\end{tabular}% close resizebox
}
\label{tab:alphashift}
\end{table}

NN, contam
default
NN, null
contam, no weight

Relative to null sys_tot (ground truth)
apar
0.011569487626905683 +/- [0.24436773 0.22665174]
-0.07366002080733125 +/- [0.23648763 0.22690789]
-6.940277930134187e-06 +/- [0.11187177 0.10279328]
0.00999973264396159 +/- [0.19959853 0.22847554]


aper
0.08388423184167992 +/- [0.16504684 0.16688782]
0.016823116081909895 +/- [0.16027468 0.16612681]
0.14818153577905724 +/- [0.08140876 0.07306003]
-0.10764608590896341 +/- [0.15945608 0.1620402 ]

